An Approximate Bayesian Long Short-Term Memory Algorithm for Outlier Detection

Long Short-Term Memory networks trained with gradient descent and back-propagation have received great success in various applications. However, point estimation of the weights of the networks is prone to over-fitting problems and lacks important uncertainty information associated with the estimation. However, exact Bayesian neural network methods are intractable and non-applicable for real-world applications. In this study, we propose an approximate estimation of the weights uncertainty using Ensemble Kalman Filter, which is easily scalable to a large number of weights. Furthermore, we optimize the covariance of the noise distribution in the ensemble update step using maximum likelihood estimation. To assess the proposed algorithm, we apply it to outlier detection in five real-world events retrieved from the Twitter platform.

==> section/acknowledgment.tex <==
%ACKNOWLEDGMENTS are optional
\section{Acknowledgments}
This section is optional; it is a location for you
to acknowledge grants, funding, editing assistance and
what have you.  In the present case, for example, the
authors would like to thank Gerald Murray of ACM for
his help in codifying this \textit{Author's Guide}
and the \textbf{.cls} and \textbf{.tex} files that it describes.


==> section/literature_review.tex <==
\section{Background}
%-------------------------------------------------------------------------------
Traditionally, unsupervised models and supervised models have been widely applied to detect events from news sources. Clustering methods have been a classic approach for both Retrospective Event Detection (RED) and New Event Detection (NED) since 1990s. According to Allan et al.~\cite{allan2002}, they designed a single pass clustering method with a threshold model to detect and track events from a collection of digitalized news sources. Chen and Roy~\cite{chen2009} also applied clustering approaches such as DBSCAN to identify events for other user-generated contents such as photos. 

Later, Sankaranarayanan et al.~\cite{sankaranarayanan2009} developed an online clustering algorithm named ''leader-follower'' to group tweets into different topics. To form high-quality clusters, they filtered out junk tweets, got rid of noisy clusters, and then combined fragmented and duplicate clusters into one master cluster sharing the same topic. Taking emotional states into considerations, Valkanas and Gunopoulos~\cite{valkanas2013} built an intelligent system that applied hierarchical clustering methods to group users based upon geographic locations and they then captured events once the cumulative emotion within the clusters fluctuated. In another experiment, Weng and Lee~\cite{weng2011} designed a system named EDCoW which first applied wavelet analysis to obtain new features for each word and then clustered remained words with high signal auto-correlation using a modularity-based graph partitioning algorithm. 

In addition to event detection, topic modeling or trend detection are related terms that are often discussed in the literature with a focus on the content. According to Mathioudakis and Koudas~\cite{mathioudakis2010}, they implemented the first research-oriented system to detect trends by grouping a set of bursty keywords using their custom algorithms. Specifically, they coined co-occurred keywords as bursty words when their tweeting rates changed, and then they grouped these keywords to identify trends. In contrast, Cataldi et al.~\cite{cataldi2010} designed a new metric to detect emerging terms with an integration of a novel aging cycle theory and the authority of sources. Then they formed a topic graph by connecting the emerging terms with other terms and extracted the trending topics as the strongly connected components. 

Aside from clustering approaches, a number of supervised algorithms have also been proposed for event detection, including naive Bayes~\cite{becker2011, sankaranarayanan2009}, SVM~\cite{sakaki2010}, and gradient boosted decision trees~\cite{popescu2010}. Becker et al.~\cite{becker2011} employed the Naïve Bayes classifier to label the clustered tweets into event-tweets or non-events tweets with derived temporal features, social features, topical features, and Twitter-centric features, while the tweets are grouped using an incremental clustering algorithm. Sakaki et al.~\cite{sakaki2010} applied the Support Vector Machine to classify tweets into tweets related to target events or not with three key features. Subsequently, they designed a spatial-temporal model to estimate the center of an earthquake and forecast the trajectory of a hurricane using Kalman Filtering and Particle Filtering. Popescu and Pennacchiotti~\cite{popescu2010} proposed a gradient boosted decision tree based model integrated with a number of custom features to detect controversial events from Twitter streams. 

Besides clustering and classification approaches, there also exist other perspectives including ensemble approaches to address the event detection problem. Sankaranarayanan et al.~\cite{sankaranarayanan2009} first employed a classification scheme to classify tweets into different groups, and then applied a clustering algorithm to identify events. Shamma et al.~\cite{shamma2009} proposed a simple statistic-based model to identify events based upon user activities, particularly to say, Twitter volume change over time. Similarly, Zhao et al.~\cite{zhao2011} claimed that their novel system could detect NFL events by exploring post rate change within an adaptive time moving window with high accuracy and prompt response. In the following analysis, they explored the event content with an extraction of top keywords based upon lexicon analysis. 

Based upon the event detection literature, there are several relevant aspects involved in the studies, such as sub-event detection, large scale analysis~\cite{petrovic2010}, event visualization~\cite{marcus2011, oconnor2010}, and event summary~\cite{zubiaga2012, chakrabarti2011, nichols2012}. 





As argued by Meladianos et al.~\cite{meladianos2015}, sub-event detection has been receiving more and more attention from the research community. A the time being, there are a number of studies dealing with sub-event detection in an offline mode~\cite{zubiaga2012, petrovic2010}. Zhao et al.~\cite{zhao2011} adopted a simple statistical approach to detect sub-events during NFL games when tweeting rate suddenly rose higher than a prior threshold. Chakrabarti and Punera~\cite{chakrabarti2011} developed a two-phase model with a modified Hidden Markov Model to identify sub-events and then derived a summary of the tweets stream. However, their approach has a severe deficiency because it fails to work properly under situations when unseen event types are involved. Zubiaga et al.~\cite{zubiaga2012} compared two different approaches for sub-event detection. The first approach measured recent tweeting activities and identified sub-events if there was a sudden increase of the tweeting rate by at least 1.7 compared to the previous period. The second approach relied on all previous tweeting activities and detected sub-events if the tweeting rate within 60 seconds exceeded 90\% of all previously tweeting rates. As claimed by the authors, the latter outlier-based approach outperformed the first increase-based approach since it neglected situations when there existed low tweeting rates preceded by even lower rates~\cite{zubiaga2012}.

Nichols et al.~\cite{nichols2012} provided both an online approach and an offline approach to detect sub-events as well as summarizing important events moments by comparing slopes of statuses updates with a specific slope threshold, which was defined as the sum of the median and three times the standard deviation (median + 3*standard deviation) in their experiment. Shen et al.~\cite{shen2013} incorporated ''burstiness'' and ''cohesiveness'' properties of tweets into a participant-based sub-event detection framework, and developed a mixture model tuned by EM which yielded the identification of important moments of an event. Chierichetti et al.~\cite{chierichetti2014} proposed a simple linear classifier, particularly to say, a logistic regression classifier, to capture the new sub-events with the exploration of the tweet and retweet rates as the features. 

In this study, we formalize sub-event detection as an outlier detection problem, and solve the problem in a novel way with a set of statistical models including Kalman Filter (KF), Gaussian Process (GP), and Probabilistic Principle Component Analysis (PPCA). 

(At the initial stage of our study, we investigated a number of features, such as number of tweets (\texttt{num\_of\_tweets}), number of users (\texttt{num\_of\_users}), log transformed of them (\texttt{log(num\_of\_tweets)}), ratio change of number of tweets (\texttt{ratio\_change}), and user engagement (\texttt{user\_engagement}). Specific, user engagement is defined as the number of tweets over the number of counts within each time window and 0 otherwise. However, these features can only be applied in our Gaussian-assumed models with certain transformation, such as relying on the corresponding residuals after trend decomposition, and thus they can only be applied in an offline mode. In our later experiments, we solely investigate the performance of \texttt{ratio\_change} in different models.)

Our first model is KF, integrated with a Kalman Filter Smoother (KFS) and Expectation Maximization (EM) to estimate the optimized parameters. The rest models include GP and PPCA, both of which predict the fourth value with the previous three consecutive value. To identify the outliers, we experimented both the 0.025 significance level and the 0.005 significance level for the one-tail test. However, we observed many false positives and decided to utilize the stricter 0.005 as the detection threshold. Later on, we incorporated the \texttt{num\_of\_tweets} as a threshold and only considered it as an outlier if the corresponding \texttt{num\_of\_tweets} was not less than 30. In terms of this refinement, we removed many false-positives and resulted in outliers matching the experimental datasets.

